Symmetric Khovanov--Rozansky link homologies

We provide a finite dimensional categorification of the symmetric evaluation of $\mathfrak{sl}_N$-webs using foam technology. As an output we obtain a symmetric link homology theory categorifying the link invariant associated to symmetric powers of the standard representation of $\mathfrak{sl}_N$. In addition, the construction is actually made in an equivariant setting. We prove also that there is a spectral sequence from the Khovanov-Rozansky triply graded link homology to the symmetric one and provide along the way a foam interpretation of Soergel bimodules.

==> _region_.tex <==
\message{ !name(sym_twistingforkplus.tex)}
\message{ !name(sym_twistingforkplus.tex) !offset(-2) }
\begin{scope}[font= \tiny]
  \coordinate (T) at (0, 1);
  \coordinate (M) at (0, 0);
  \coordinate (B1) at (-1, -1);
  \coordinate (B2) at (1, -1);
  \draw[->] (M) -- (T) node[above] {$a+b$};
  \draw[->-] (B1)  node[below] {$a$} .. controls +( 0.1, 0.1) and +( 0.5 ,-0.3) .. (M);
  \fill[yellow] (0,-0.5) circle (0.1);
  \draw[->-] (B2)  node[below] {$b$} .. controls +(-0.1, 0.1) and +(-0.5 ,-0.3) .. (M);
\end{scope}
\message{ !name(sym_twistingforkplus.tex) !offset(-13) }


==> categorification.tex <==

% \subsection{Universal construction}
% \label{sec:univ-constr}
% \input{uc}

% \subsection{A foamy interpretation of Soergel bimodules}
% \label{sec:soergel-bimodules}
% \input{soergel}

% \subsection{Hochschild homology via foams}
% \label{sec:hochsch-homol-via}
% \input{hochschild}

% \subsection{Categorification of the symmetric MOY calculus}
% \label{sec:symm-moy-calc}
% % \todo{
% \begin{itemize}
% \item Theorème: catégorification, il faut peut être un nom pour le type de TQFT: \emph{tube-like} ? 
% \item Preuve: on réduit en mode exterieure, cercles concentrique.
% \end{itemize}
% }

%\input{catsym}

% \subsection{HOMFLYPT-homology}
% \label{sec:uncol-symm-gll_n}





%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "sym"
%%% End: 


==> hochschild.tex <==
 
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "sym"
%%% End: 


==> llanglerrangle.tex <==
\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}%
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}%
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother


==> sym_GammaCircle.tex <==
\begin{scope}[xscale=-1]
%\node at (180: 4) {$\Gamma_1:=$}
\filldraw[fill=blue!20!white, draw = black] (-145:1.45) arc (-145:145:1.45) -- +(145:1.6) arc (145: -145:3.05) -- cycle;
\draw[green!50!black, thick,->] (-145:1.5) arc (-145:-215:1.5) node[left, midway] {\tiny{$1$}}; 
\draw[->] (-145:2) arc (-145:-215:2);
%\draw (-145:2.5) arc (-145:-215:2.5); 
\node at (180:2.5) {$\dots$};
\node at (0:2.25) {$\Gamma$};
\draw[->] (-145:3) arc (-145:-215:3);
\draw[blue!50!black, thick,->] (145:1) arc (145:-215:1) node[right, midway] {\tiny{$1$}}; 
%\draw (-150:1) arc (-150:150:1)  .. controls +(-120:0.2) and +(80:0.2) .. (170:1.25)  arc (170:190:1.25)
%.. controls +(-80:0.2) and +(120:0.2 ) .. (-150:1);
% -- +(145:1.6) arc (145: -145:3.05) -- cycle;
\end{scope}


==> sym_MPsplit.tex <==
%\begin{scope}
% \draw[->] (0,0) -- (0,0.5) node [at end, above] {$a+b$};  
% \draw[>-] (-0.5, -0.5) -- (0,0) node [at start, below] {$a$};  
% \draw[>-] (+0.5, -0.5) -- (0,0) node [at start, below] {$b$};  
\begin{scope}[yscale = 1]
\coordinate (O) at (0,0) node [below] {$a+b+c$};
\coordinate (O1) at (0,1);
\coordinate (O2) at (1,2);
\coordinate (A) at (-2,3); %node [above] {$a$};
\coordinate (B) at (0,3);  %node [above] {$b$};
\coordinate (C) at (2,3);  %node [above] {$c$};
\draw[>-] (O) -- (O1); 
\draw[->] (O1) -- (O2);
\draw[->] (O1) -- (A) node [above] {$a$};
\draw[->] (O2) -- (B) node [above] {$b$};
\draw[->] (O2) -- (C) node [above] {$c$}; 
\end{scope}
\node at (3.5, 1.5) {$=$};
\begin{scope}[xshift = 7cm]
\coordinate (O) at (0,0) node [below] {$a+b+c$};
\coordinate (O1) at (0,1);
\coordinate (O2) at (-1,2);
\coordinate (A) at (-2,3); %node [above] {$a$};
\coordinate (B) at (0,3); %node [above] {$b$};
\coordinate (C) at (2,3); %node [above] {$c$};
\draw[>-] (O) -- (O1); 
\draw[->] (O1) -- (O2);
\draw[->] (O1) -- (C) node [above] {$c$};
\draw[->] (O2) -- (B) node [above] {$b$};
\draw[->] (O2) -- (A) node [above] {$a$};
\end{scope}


==> sym_digon.tex <==
%\begin{scope}
% \draw[->] (0,0) -- (0,0.5) node [at end, above] {$a+b$};  
% \draw[>-] (-0.5, -0.5) -- (0,0) node [at start, below] {$a$};  
% \draw[>-] (+0.5, -0.5) -- (0,0) node [at start, below] {$b$};  
\begin{scope}[yscale = 1]
\coordinate (O1) at (0,0) node [below] {$a+b$};
\coordinate (O2) at (0,1);
\coordinate (O3) at (0,3);
\coordinate (O4) at (0,4);
\draw[>-] (O1) -- (O2);
\draw[->] (O2) .. controls + (-1, 1).. (O3) node [midway,left] {$a$};
\draw[->] (O2) .. controls + ( 1, 1).. (O3) node [midway,left] {$b$};
%\draw[->] (O2) -- (O3) node [above] {$b$};
\draw[->] (O3) -- (O4) node [above] {$a+b$}; 
\end{scope}
\node at (3, 2) {$= \
\begin{bmatrix}
  a+b \\
  a\,\,\,\,b
\end{bmatrix}
$};
\begin{scope}[xshift = 5cm]
\coordinate (O1) at (0,0) node [below] {$a+b$};
\coordinate (O4) at (0,4);
\draw[->] (O1) -- (O4) node [above] {$a+b$}; 
\end{scope}


==> sym_doubledigon.tex <==
\begin{scope}[yscale =0.6]
\begin{scope}
  \coordinate (AR) at (-90:2);
  \coordinate (BR) at ( 90:2);
  \draw[-<-] (-90:2) arc (-90:-45:2);% node[below, left] {$N$};
  \draw[-<-] (-45:2) arc (-45:-35:2);% node[below, left] {$N$};
  \draw[densely dotted] (-35:2) arc (-35:-20:2);% node[below, left] {$N$};
  \draw[-<-] (-20:2) arc (-20:20:2)  node[midway, right] {$k_l$};
  \draw[densely dotted] (20:2) arc (20:35:2);% node[below, left] {$N$};
  \draw[-<-] (35:2) arc (35:45:2);% node[below, left] {$N$};
  \draw[-<-] (45:2) arc (45:90:2);% node[] {$N$};
%
  \node at (1.5, 0) {$\dots$};
  \draw[-<-] (-20:2) arc (200:160:2);% node[below, left] {$N$};
  \draw[-<-] (-35:2) arc (215:145:2);% node[below, left] {$N$};
  \draw[-<-] (-45:2) arc (225:135:2) node[midway, left] {$k_1$};
\end{scope}

\begin{scope}[xshift = -3, xscale = -1]
  \coordinate (AL) at (-90:2);
  \coordinate (BL) at ( 90:2);
  \draw[->-] (-90:2) arc (-90:-45:2);% node[below, left] {$N$};
  \draw[->-] (-45:2) arc (-45:-35:2);% node[below, left] {$N$};
  \draw[densely dotted] (-35:2) arc (-35:-20:2);% node[below, left] {$N$};
  \draw[->-] (-20:2) arc (-20:20:2) node[midway, left] {$k_l$};% node[below, left] {$N$};
  \draw[densely dotted] (20:2) arc (20:35:2);% node[below, left] {$N$};
  \draw[->-] (35:2) arc (35:45:2);% node[below, left] {$N$};
  \draw[->-] (45:2) arc (45:90:2);% node[] {$N$};
%
  \node at (1.5, 0) {$\dots$};
  \draw[-<-] (-20:2) arc (200:160:2);% node[below, left] {$N$};
  \draw[->-] (-35:2) arc (215:145:2);% node[below, left] {$N$};
  \draw[->-] (-45:2) arc (225:135:2) node[midway, right] {$k_1$};
\end{scope}

\draw (AR) -- (AL) node[midway, above] {$N$};
\draw (BR) -- (BL) node[midway, below] {$N$};

\end{scope}


%  \draw[->-] (135:2) arc (135:225:2) node[midway, right] {$k_1$};

==> sym_examplevinyltalk.tex <==
\begin{scope}
  \coordinate (O) at (0, 0);
  \fill[yellow] (O) circle (4cm);
  \fill[white] (O) circle (2cm);
  \draw[dotted] (O) circle (2cm);
  \draw[dotted] (O) circle (4cm);
  \coordinate (F1) at (30:3.8);
  \coordinate (F2) at (90:3.8);
  \coordinate (F3) at (-45:3.8);
  \coordinate (M1) at (135:3);
  \coordinate (M2) at (-90:3);
  \coordinate (M3) at (-45:3);
  \coordinate (I1) at (90:2.2);
  \coordinate (I2) at (180:2.2);
  \coordinate (I3) at (225:2.2);
  \coordinate (I4) at (-90:2.2);
  %\draw[->-] (O) circle (2.2cm);
  \draw[->-] (I1) arc (90:180:2.2);  %node[midway, right] {$1$};
  \draw[->-] (I2) arc (180:225:2.2); % node[midway, right] {$6$};
  \draw[->-] (I3) arc (-135:-90:2.2); % node[midway, above] {$4$};;
  \draw[->-] (I4) arc (-90:90:2.2); %node[midway, left] {$2$};
  %\draw[->] (O) circle (3.8cm);
  \draw[->-] (M3) .. controls +(45:0.5) and +(-60:0.5) .. (F1);% node[midway, right] {$3$};
  \draw[->-] (F2) .. controls +(180:0.5) and +(45:0.5) .. (M1) ;% node[midway, right] {$4$};
  \draw[->-] (I1) .. controls +(180:0.5) and +(45:0.5) .. (M1);% node[midway, above] {$1$};
  \draw[->-] (M1) .. controls +(225:0.5) and +(90:0.5) .. (I2) ;% node[midway, right] {$5$};
  \draw[->-] (I3) .. controls +(-45:0.5) and +(180:0.5) .. (M2) ;% node[midway, below] {$2$};
  \draw[->-] (I4) .. controls +(0:0.5) and +(225:0.5) .. (M3) ;% node[near end, above] {$2$};
  \draw[->-] (M2) .. controls +(0:0.5) and +(225:0.5) .. (M3);% node[near start, above] {$1$};
  \draw[->-] (M2) .. controls +(0:0.5) and +(225:0.5) .. (F3) ;% node[near end, above] {$1$};
  \draw[->-] (F1) .. controls +(120:1.5) and +(0:1.5) .. (F2) ;% node[midway, right] {$5$};
  \draw[->-] (F2) .. controls +(180:1.5) and  +(70:1) .. (160:3.5) .. controls +(250:1.5) and +(135:1.5) .. (225:3.5) % node[left] {$1$} 
.. controls +(-45:1.5) and +(225:1.5) .. (F3);
  \draw[->-] (F3) .. controls +(45:1.5) and +(-60:1.5) .. (F1) ;% node[midway, right] {$2$};
\end{scope}

==> sym_gendigon.tex <==
\tdplotsetmaincoords{60}{140}
\begin{scope}[tdplot_main_coords]
  \coordinate (aT) at (-1, 0, 2);
  \coordinate (bT) at (+1, 0, 2);
  \coordinate (AT) at (-2.5, 0, 2);
  \coordinate (BT) at (+2.5, 0, 2);
  \coordinate (cT) at (0, +1, 2);
  \coordinate (dT) at (0, -1, 2);
  \coordinate (aB) at (-1, 0, -2);
  \coordinate (bB) at (+1, 0, -2);
  \coordinate (AB) at (-2.5, 0, -2);
  \coordinate (BB) at (+2.5, 0, -2);
  \coordinate (cB) at (0, +1, -2);
  \coordinate (dB) at (0, -1, -2);
  \coordinate (aM) at (-1, 0, 0);
  \coordinate (bM) at (+1, 0, 0);
\draw[thick, -<-] (AT) -- (aT);
\draw[thick, -<-] (bT) -- (BT);
\draw[thick, -<-] (aT) .. controls (dT) .. (bT);
\draw[thick, -<-] (aT) .. controls (cT) .. (bT);
\draw[thick, -<-] (AB) -- (aB);
\draw[thick, -<-] (bB) -- (BB);
\draw[thick, -<-] (aB) .. controls (dB) .. (bB);
\draw[thick, -<-] (aB) .. controls (cB) .. (bB);
\draw[thick, -<-] (aB) -- (aT);
\draw[thick, -<-] (bT) -- (bB);
  \filldraw[draw = black, rounded corners=1pt, thick, fill opacity = 0.3, fill = red]    (AT) -- (aT) node[pos=0.65, opacity =1, below, sloped] {$\scriptstyle{a+b}$} -- (aB) -- (AB) -- (AT);
  \filldraw[draw = black, rounded corners=1pt, thick, fill opacity = 0.3, fill = red]    (bT) -- (BT) node[pos=0.65, opacity =1, below, sloped] {$\scriptstyle{a+b}$} -- (BB) -- (bB) -- (bT);
  \filldraw[draw = black, rounded corners=1pt, thick, fill opacity = 0.3, fill = blue]   (bT) .. controls (dT) .. (aT) node[near end, below, opacity=1] {$\scriptstyle{a}$} -- (aB) .. controls (dB) .. (bB)-- (bT);
  \filldraw[draw = black, rounded corners=1pt, thick, fill opacity = 0.3, fill = green]   (bT) .. controls (cT) .. (aT) -- (aB)  .. controls (cB) .. (bB) node[near end, above= -0.1cm, opacity=1] {$\scriptstyle{b}$} -- (bT);



\end{scope}

==> sym_idSkP.tex <==
\begin{scope}
  \draw[->-] (-2,0) arc (180:360: 2cm and 1cm) node[midway, above] {$k$};
  \draw[dashed] (-2,0) arc (180:0: 2cm and 1cm);
  \draw (-2,3) arc (180:360: 2cm and 1cm);
  \draw[-<-] (-2,3) arc (180:0: 2cm and 1cm)  node[midway, below] {$k$};
  \node[red, very thick] at (0, 1.5) {$P$};
  \draw (2,0) -- +(0,3);
  \draw (-2,0) -- +(0,3);
\end{scope}

==> sym_wave_inject.tex <==
\begin{scope}
  \coordinate (A1) at (0, 1);
  \coordinate (A2) at (2, 2);
  \coordinate (B1) at (0, 2);
  \coordinate (B2) at (2, 3);
  \coordinate (C1) at (1, 3.5);
  \coordinate (C2) at (3, 4.5);
  \coordinate (D1) at (-0.5, 4);
  \coordinate (D2) at ( 1.5, 5);
\filldraw[thick, draw = black, fill=red, fill opacity = 0.4] (A1)-- (A2) -- (B2) -- (B1) -- cycle;
\filldraw[thick, draw = black, fill=blue, fill opacity = 0.4] (D1)-- (D2) .. controls +(0,0) and +(0, 0.5) .. (B2) -- (B1)  .. controls +(0,0.5) and +(0, 0) .. cycle;
\filldraw[thick, draw = black, fill=green, fill opacity = 0.4] (C1)-- (C2) .. controls +(0,0) and +(0, 0.5) .. (B2) -- (B1)  .. controls +(0,0.5) and +(0, 0) .. cycle;
\end{scope}
\node at (3.3,2.5) {$\rightsquigarrow$};
\begin{scope}[xshift = 5cm]
  \coordinate (A1) at (0, 1);
  \coordinate (A2) at (2, 2);
  \coordinate (B1) at (0, 2);
  \coordinate (B2) at (2, 3);
  \coordinate (C1) at (1, 3.5);
  \coordinate (C2) at (3, 4.5);
  \coordinate (D1) at (-0.5, 4);
  \coordinate (D2) at ( 1.5, 5);
  \coordinate (E) at ( 1, 3.3);
  \filldraw[thick, draw = black, fill=red, fill opacity = 0.4] (A1)-- (A2) --  (B2)  .. controls +(-0.5, -0.25) and +(0.5,0.25 ) .. (E)  .. controls +(-0.5,-0.25) and +(0.5, 0.25 ) ..  (B1) -- cycle;
\filldraw[thick, draw = black, fill=blue, fill opacity = 0.4] (D1)-- (D2) .. controls +(0,0) and +(0, 0.5) .. 
(B2)  .. controls +(-0.5, -0.25) and +(0.5,0.25 ) .. (E)  .. controls +(-0.5,-0.25) and +(0.5, 0.25 ) ..  (B1)
.. controls +(0,0.5) and +(0, 0) .. cycle;
\filldraw[thick, draw = black, fill=green, fill opacity = 0.4] (C1)-- (C2) .. controls +(0,0) and +(0, 0.5) .. 
(B2)  .. controls +(-0.5, -0.25) and +(0.5,0.25 ) .. (E)  .. controls +(-0.5,-0.25) and +(0.5, 0.25 ) ..  (B1)
.. controls +(0,0.5) and +(0, 0) .. cycle;
\end{scope}

==> symev.tex <==


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "sym"
%%% End: 


==> symslninvariant.tex <==

The aim of this section is to fix notations and to recall the definition of the quantum link invariant associated with the symmetric powers of the quantum groups $U_q(\sll_N)$. In what follows $q$ is a generic indeterminate. 

\subsection{Representations of $U_q(\gll_N)$}
\label{sec:repr-gll_n}

\marginpar{Faut-il parler de  $\sll_N$ ou $\gll_N$. Je pense que c'est meux de se placer dans le cadre $\gll_N$, mais je n'ai pas de référence sur les représentations...}
\begin{dfn}[\cite{kassel97:_quant}]  \label{dfn:Uqsln}
  The associative $\CC(q)$-algebra generated by $E_i, F_i, K_i, K^{-1}_i$ for $i$ in $\llbracket 1, n-1$ and submitted to the relations
\[
BLABLA
 \] is denoted $U_q(\gll_N)$. The following definition of co-unit and co-multiplication endow it with a structure of BLABLA quasi-triangular Hopf algebra:
\[
BLABLA
\]
\end{dfn}

The algebra $U_q(\gll_N)$ is a deformation of $U(\gll_N)$, the universal enveloping algebra of the Lie algebra $\gll_N$. It is well-known that its finite dimensional modules\footnote{We only consider modules of type $+1$. Those are weight modules where the actions of the $K_i$ can be diagonalised and have weight of the form $q^b$ for some integers $b$. All finite dimensional $U_q(\gll_N)$-modules are weight modules, but the weight have the form $\pm q^b$.   } are deformation of the finite dimensional $\sll_N$-modules. We denote by $V$ the $U_q(\gll_N)$-modules which is the deformation (of type $+1$) 


\todo{
\begin{itemize}
\item Parler de R matrice. Invariant d'entrelacs
\item Parler des toiles exterieures ? Ca peut être un peu confusing, mais ce serait bien quand même quand on parlera ,de la catégorification des exterieures. A cause du problème de signe on a pas de toile mixe.
\item dictionnaire avec les diagramme
\item Citer \cite{tubbenhauer2015super} pour les toiles mixtes
\end{itemize}
}


\subsection{MOY calculus for symmetric webs}
\label{sec:moy-calc-symm}

\todo{
\begin{itemize}
\item Formules exterieures
\item Formules exterieures
\item remarque  sur le signes / lien avec le changement de tressage / dualité de Koszule / dualité Boson-Fermion HAHAHA !
\item braids-like graphs.
\item Proposition somme d'états.
\item lemme: Arbre 
\end{itemize}
}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "sym"
%%% End: 


==> uc.tex <==
The universal construction is a procedure which under favorable circumstances extend an invariant of closed cobordisms\footnote{These are cobordisms from the empty set to the emtpy set.} to a TQFT functor. Except from the cas $r=0$, the empty set is not an object of $\TL_r$, so we need a replacement for the notion of closed cobordisms. This role will be played by the endomorphisms of the circle labeled by $r$ which we denote from now on $\mathcal{S}_r$. Before we describe the $N$th evaluation of the elements of $\mathrm{Hom}_{\TL_r}(\mathcal{S}_r, \mathcal{S_r})$, we need to introduce the map
\[
  \begin{array}{crcl}
    \phi_{r,N}:& \ZZ[X_1, \dots, X_k]^{\mathfrak{S}_k} & \to &\ZZ \\
& \displaystyle{\sum _{\lambda \textrm{Young diagram}} a_\lambda \pi_\lambda} &\mapsto & a_{\rho(k, N-1)}.
  \end{array}
\]
and the 

\begin{dfn}
  Let $F$ be an element of $\mathrm{Hom}_{\TL_r}(\mathcal{S}_r, \mathcal{S}_r)$. We denote by $\widehat{F}$, the closed foam obtained by gluing on $F$ two disks labeled $k$.  
  The symmetric evaluation $\kup{F}_S^N$ of the tube-like $\mathcal{S}_r$-foam-$\mathcal{S}_r$ $F$ is defined to be equal to $\phi_{r,N}(\kup{\widehat{F}}_r)$.
\end{dfn}

We are now in position to apply the universal construction.  If $\Gamma$ is an object of $\TL_r$, we define
\[
\widetilde{V}(\Gamma) = \left(\bigoplus_{F\in \mathrm{Hom}_{\TL_r}(\mathcal{S}_r, \Gamma)} \ZZ\right)\{- k(N-1)\}.
\] 
Note that $\widetilde{V}(\Gamma)$ inherits a grading from the degree of tube-like foams.
If $\Gamma_1$ and $\Gamma_2$ are two objects of $\TL_r$ and $F$ is an element of $\mathrm{Hom}_{\TL_r}(\Gamma_1, \Gamma_2)$, we define the $\ZZ$-module map
\[
    \widetilde{W}(F) : \widetilde{V}(\Gamma_1)   \to  \widetilde{V}(\Gamma_2)
\]
on the base of $\widetilde{V}(\Gamma_1)$ by the following formula:
\[
     \widetilde{W}(F)(G) = F\circ G.
\]
where $G$ is an element of $\mathrm{Hom}_{\TL_r}(\mathcal{S}_r, \Gamma_1)$ and the composition is the composition of $\TL_r$. 

No we use the evaluation of symmetric foams to mod out. 
For all $F'$ in $\mathrm{Hom}_{\TL_r}(\Gamma, \mathcal{S}_r)$, we define the $\ZZ$-linear map
\[
  \begin{array}{crcl}
    \tau_F':  & \widetilde{V}(\Gamma)& \to & \ZZ \\
& F&\mapsto & \kup{F'\circ F} _{S}^N
  \end{array}
\]
We define
\[
\mathcal{F}_{r,N}(\Gamma)=\widetilde{\Gamma}\left/ \bigcap_{F' \in \mathrm{Hom(\Gamma, \mathcal{S}_r)}} \mathrm{Ker} (\tau_F')\right..
\] 

If $F$ is an element of $\mathrm{Hom}_{\TL_r}(\Gamma_1, \Gamma_2)$, the map $\widetilde{W}(F)$ induces a $\ZZ$-linear map from $\mathcal{F}_{r,N}(\Gamma_1)$ to $\mathcal{F}_{r,N}(\Gamma_2)$ which we denote  by $\mathcal{F}_{r,N}(F)$

\begin{prop}
  The above construction of $\mathcal{F}_{r,N}$ gives rise to a functor from $\TL_r$ to the category of graded $\ZZ$-modules. 
\end{prop}

The proof is straight forward, a similar argument is developed in \cite[BLABLA]{RW1}.

\begin{thm}\label{thm:catMOY}
  The functors $\left(\mathcal{F}_{r,N}\right)_{r\in \NN}$ categorifiy the symmetric MOY calculus for braid-like graphs.
\end{thm}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "sym"
%%% End: 

